Approximate Contraction of Arbitrary Tensor Networks with a Flexible and Efficient Density Matrix Algorithm

Tensor network contractions are widely used in statistical physics, quantum computing, and computer science. We introduce a method to efficiently approximate tensor network contractions using low-rank approximations, where each intermediate tensor generated during the contractions is approximated as a low-rank binary tree tensor network. The proposed algorithm has the flexibility to incorporate a large portion of the environment when performing low-rank approximations, which can lead to high accuracy for a given rank. Here, the environment refers to the remaining set of tensors in the network, and low-rank approximations with larger environments can generally provide higher accuracy. For contracting tensor networks defined on lattices, the proposed algorithm can be viewed as a generalization of the standard boundary-based algorithms. In addition, the algorithm includes a cost-efficient density matrix algorithm for approximating a tensor network with a general graph structure into a tree structure, whose computational cost is asymptotically upper-bounded by that of the standard algorithm that uses canonicalization. Experimental results indicate that the proposed technique outperforms previously proposed approximate tensor network contraction algorithms for multiple problems in terms of both accuracy and efficiency.

==> kdt_misc.tex <==
\begin{lem}
    Let $\tau$ be a permutation of $\sigma$ and the subset $\hat{C}\subset C$ with $|\hat{C}|=n$. $\tau$ has a constraint that values in $\hat{C}$ are assigned to indices $\hat{I} = \{i_1,\ldots,i_n\}$. When $\tau[\hat{C}] = \sigma[\hat{C}]$, we have $\tau$ minimizes $\min_{\tau}\ktdist{\sigma,\tau}$.
\end{lem}
\begin{proof}
    Consider two rankings under the constraint, $\tau_1,\tau_2$, where $\tau_1[C\setminus\hat{C}]$ can be any ordering and  $\tau_1[C\setminus\hat{C}]=\tau_2[C\setminus\hat{C}]$. Below we show that when $\tau_1[\hat{C}] = \sigma[\hat{C}]$, we always have 
    $\ktdist{\sigma,\tau_1}\leq \ktdist{\sigma,\tau_2}$. This finishes the proof.

For two sets $S_1,S_2\subseteq C$, let 
\[
\beta(S_1,S_2) = \sum_{c\in S_1,c'\in S_2, c< c'} 
\mathbbm{1}\Big(\sigma(c,c')\neq \tau_2(c,c')\Big) - 
\mathbbm{1}\Big(\sigma(c,c')\neq \tau_1(c,c')\Big),
\]
we have
\begin{align*}
    \ktdist{\sigma,\tau_2} - \ktdist{\sigma,\tau_1} = \beta(C,C)\\
    = \beta(C\setminus\hat{C},C\setminus\hat{C}) + 
    \beta(\hat{C}, \hat{C}) + 
\beta(C\setminus\hat{C},\hat{C}) + 
\beta(\hat{C},C\setminus\hat{C}) \\
= \beta(\hat{C}, \hat{C}) + 
\beta(C\setminus\hat{C},\hat{C}) + 
\beta(\hat{C},C\setminus\hat{C}).
\end{align*}
Based on the definition, $\beta(\hat{C}, \hat{C}) \geq 0$. 
Below we consider $\beta(C\setminus\hat{C},\hat{C}) + 
\beta(\hat{C},C\setminus\hat{C}).$

Consider the case where $|\hat{C}|=2$, and we denote $\hat{C} = \{a,b\}$ with $\sigma(a)<\sigma(b)$. Let $C_L = \{c\in C\setminus \hat{C}, \sigma(c)<\sigma(a)\}$, $C_M = \{c\in C\setminus \hat{C}, \sigma(a)<\sigma(c)<\sigma(b)\}$, and let $C_G = \{c\in C\setminus \hat{C}, \sigma(c)>\sigma(b)\}$.
For this case,
\begin{align*}
    \beta(C\setminus\hat{C},\hat{C}) + 
\beta(\hat{C},C\setminus\hat{C}) = \sum_{c\in C_L,c'\in \hat{C}} 
\mathbbm{1}\Big(\sigma(c,c')\neq \tau_2(c,c')\Big) - 
\mathbbm{1}\Big(\sigma(c,c')\neq \tau_1(c,c')\Big) \\
+ \sum_{c\in C_M,c'\in \hat{C}} 
\mathbbm{1}\Big(\sigma(c,c')\neq \tau_2(c,c')\Big) - 
\mathbbm{1}\Big(\sigma(c,c')\neq \tau_1(c,c')\Big) \\
+ \sum_{c\in C_G,c'\in \hat{C}} 
\mathbbm{1}\Big(\sigma(c,c')\neq \tau_2(c,c')\Big) - 
\mathbbm{1}\Big(\sigma(c,c')\neq \tau_1(c,c')\Big).
\end{align*}
We have $\tau_2(c,a) = \tau_1(c,b)$ and $\tau_2(c,b) = \tau_1(c,a)$. 
When $c\in C_L$, we have the equation above equals
\begin{align*}
    \sum_{c\in C_L} 
\mathbbm{1}\Big(\sigma(c,a)\neq \tau_2(c,a)\Big) + \mathbbm{1}\Big(\sigma(c,b)\neq \tau_2(c,b)\Big) - 
\mathbbm{1}\Big(\sigma(c,a)\neq \tau_1(c,a)\Big)
-
\mathbbm{1}\Big(\sigma(c,b)\neq \tau_1(c,b)\Big) \\
=     \sum_{c\in C_L} 
\mathbbm{1}\Big(\sigma(c,a)\neq \tau_1(c,b)\Big) + \mathbbm{1}\Big(\sigma(c,b)\neq \tau_1(c,a)\Big) - 
\mathbbm{1}\Big(\sigma(c,a)\neq \tau_1(c,a)\Big)
-
\mathbbm{1}\Big(\sigma(c,b)\neq \tau_1(c,b)\Big).
\end{align*}
    We have $\sigma(c,a) = \sigma(c,b)=1$. Therefore, the equation above equals 0. Same case holds for $c\in C_G$.

Now let's look at when $c\in C_M$. In this case, $\sigma(c,a) =1, \sigma(c,b)=0$. When $\tau_1(c,a)=\tau_1(c,b)$, the equation above is 0. When $\tau_1(c,a)=1$ and $\tau_1(c,b)=0$, above equals
\[
\mathbbm{1}\Big(\sigma(c,a)\neq \tau_1(c,b)\Big) + \mathbbm{1}\Big(\sigma(c,b)\neq \tau_1(c,a)\Big)\geq 0.
\]
Therefore when $|\hat{C}|=2$, $\beta(C\setminus\hat{C},\hat{C}) + 
\beta(\hat{C},C\setminus\hat{C})\geq 0$.

When $|\hat{C}|>2$, for a given $\tau[\hat{C}]$, we can perform multiple permutations, each one operating on 2 elements, and making $\tau[\hat{C}]=\sigma[\hat{C}]$ without increasing the distance. This finishes the proof.
\end{proof}
% \left|
% \left\{
% (c,c')\in C\times C 
% \text{ } | \text{ }
% c <_{\tau_1} c' \wedge c' <_{\tau_2} c
% \right\}
% \right|
% \]

\begin{defn}[Directed multitree]
    A directed multitree is a directed acyclic graph (DAG) in which there is at most one directed path between any two vertices.
\end{defn}

\begin{defn}[Directed multitree for edge group propagation]
    Consider a tensor network $G=(V,E)$, a partitioning $V_1,\ldots,V_n$ and a binary grouping tree $T_g$. For each subset $V_i$, let $\hat{V}_1,\ldots, \hat{V}_{n_i}$ denote all other leaf nodes in $T_g[V_i]$. We use $T_m(V_i,T_g)$ denotes the directed multitree for edge group propagation on top of $V_i$ and $T_g$, where $E(V_i,\hat{V}_{1}),\ldots,E(V_i,\hat{V}_{n_i})$ are leaf nodes of $T_m(V_i,T_g)$, and each parent node represents the union of all its children nodes' edges. Each parent node is added only when its represented edges are contracted in $T_g[V_i]$. 
\end{defn}

 \begin{figure}[!ht]
\centering
\subfloat[]{\includegraphics[width=.15\textwidth, keepaspectratio]{draft_pic/G1.png}}
\subfloat[]{\includegraphics[width=.43\textwidth, keepaspectratio]{draft_pic/Tg1.png}}
\subfloat[]{\includegraphics[width=.37\textwidth, keepaspectratio]{draft_pic/F1.png}}

\subfloat[]{\includegraphics[width=.33\textwidth, keepaspectratio]{draft_pic/G2.png}}
\subfloat[]{\includegraphics[width=.33\textwidth, keepaspectratio]{draft_pic/Tg2.png}}
\subfloat[]{\includegraphics[width=.33\textwidth, keepaspectratio]{draft_pic/F2.png}}

\subfloat[]{\includegraphics[width=.33\textwidth, keepaspectratio]{draft_pic/G3.png}}
\subfloat[]{\includegraphics[width=.33\textwidth, keepaspectratio]{draft_pic/Tg3.png}}
\subfloat[]{\includegraphics[width=.33\textwidth, keepaspectratio]{draft_pic/F3.png}}

\caption{
}
\end{figure}



Note that $T_m(V_i,T_g)$ is a multitree rather than a tree, and each directed tree in the multitree may not be single-rooted. In addition, this may not be a binary tree.
% We can transfer each directed tree into a directed rooted tree as described below.
% The directed tree also may not be efficient since it doesn't consider the structure of input grouping. \TODO{}

\begin{defn}[Edge propagation multitree-consistent edge ordering]
Consider an edge propagation multitree and a specific propagation path based on the binary grouping path. There must exist an edge ordering such that for each node in the propagation path, either the  inputs to the node neighbor each other, or they are separated by other edges whose parent nodes are the same as one of the inputs in some previous contractions.
\end{defn}



 \begin{figure}[htb]
\centering
\subfloat[]{\includegraphics[width=.15\textwidth, keepaspectratio]{draft_pic/G1.png}}
\subfloat[]{\includegraphics[width=.43\textwidth, keepaspectratio]{draft_pic/Tg1.png}}
\subfloat[]{\includegraphics[width=.37\textwidth, keepaspectratio]{draft_pic/TGv1.png}}

\caption{
}
\end{figure}
